Bounding smooth Levi-flat hypersurfaces in a Stein manifold

This paper is concerned with the problem of constructing a smooth Levi-flat hypersurface locally or globally attached to a real codimension two submanifold in $\mathbb C^{n+1}$, or more generally in a Stein manifold, with elliptic CR singularities, a research direction originated from a fundamental and classical paper of E. Bishop. Earlier works along these lines include those by many prominent mathematicians working both on complex analysis and geometry. We prove that a compact smooth (or, real analytic) real codimension two submanifold $M$, that is contained in the boundary of a smoothly bounded strongly pseudoconvex domain, with a natural and necessary condition called CR non-minimal condition at CR points and with two elliptic CR singular points bounds a smooth-up-to-boundary (real analytic-up-to-boundary, respectively) Levi-flat hypersurface $\widehat{M}$. This answers a well-known question left open from the work of Dolbeault-Tomassini-Zaitsev, or a generalized version of a problem already asked by Bishop in 1965. Our study here reveals an intricate interaction of several complex analysis with other fields such as symplectic geometry and foliation theory.

==> s3_openness.tex <==
%\section{Openness: Local deformation of a smooth Stein hypersurface}


%In this section, we provide a proof of Theorem \ref{openness}. Let $S=\cup_{t\in(-1,1)} S_t$ be as in Theorem  \ref{openness}. Notice that, by a theorem of  Harvey-Lawson \cite{HL},  each $S_t$ bounds a complex analytic variety $\wh{S_t}$  of codimension one with possible isolated normal singularities. (Normality follows from the fact that each singularity is an isolated hypersurface singularity.) %Moreover, $\wh{S_t}$ has $S_t$ as its  $C^{N_0-2}$-smooth or real analytic boundary as we assumed that $M$ is contained in a bounded strongly pseudoconvex domain $\O$.
%By counting the dimension of the intersection of complex analytic varieties as in \cite{DTZ2}, one sees that  $\wh{S_{t_1}}\cap \wh{S_{t_2}}=\emptyset $ for $t_1\not = t_2$. For otherwise, the intersection is a complex analytic variety in $\O$  of complex dimension at least $n-1\ge 1$ that will have a non-trivial intersection with $\p \O$. By the maximum principle, each $\wh{S_t}\subset \O$, we conclude that   ${S_{t_1}}\cap {S_{t_2}}\not =\emptyset$. This is a contradiction.  


%\begin{proof}[Proof of Theorem \ref{openness}]
%Let $p_0\in S_0$. In a local holomorphic chart, we assume $\mathcal M$  near $p_0$ is an open subset of $\CC^{n+1}$ with coordinates $(z,w)=(z_1,\cdots,z_n,w)\in \CC^n\times\CC$. After a holomorphic change of coordinates,  assume $p_0=0$ and ${\rm Span}(T_{0}{S_0}\cup J(T_{0} {S_0}))$ is defined by $\{w=0\}$. %$T^{(1,0)}_0S_0=\{w=0\}$. %Here we use $(z,w)=(z_1,\cdots,z_n,w)$ for coordinates of $\CC^{n+1}$.
%Define $\pi$ the projection map of $\CC^{n+1}\ra \CC^n$ by sending
%$(z,w)$ to $z$. Then, when restricted to each $S_t$  near $p_0$, $\pi$ is a CR diffeomorphism.  Define $\Phi$ from $S$ near $p_0=0$ to the space $(-1,1)\times\CC^{n}$ by sending each $p\in S_t$ to $(t, \pi(p))$. Letting $\psi$ be as in the theorem, notice that $\psi_{*}(\frac{\p}{\p t})$ is transversal to $S_0$ at $p$ by the  hypothesis. On the other hand, let $\rho$ be a strongly plurisubharmonic defining function of $\O$ near $p_0$ and let $\xi(\tau)$ be a   holomoprhic embedding from the unit disk  $\D\subset \CC$ into $\wh{S_0}$ with its image near $p_0$,  which is $C^1$-smooth up to $\ov{\D}$  and is attached to $S_0$ in the sense that  $\xi(\p \D)\subset \p \O$. Assume that $\xi(1)=p_0$.  %the maximum principle, $\xi(\ov{\D})\subset \wh{S_0}$. 
%Applying the Hopf lemma to $\rho\circ \xi$ at $\tau=1$, $\xi_*$ maps the normal direction of $\D$ at $1$ to a normal dircetion of $\O$ at $p_0$.   We thus  conclude that $\wh{S_0}$ is transversal to $\p \O$ and thus to $S$. In particular, we see that $\psi_{*}(\frac{\p}{\p t})$ is transversal to $\wh{S_0}$ at $p_0$.
  %By the hypothesis in the theorem on the diffeomorphism of $\psi$, 
%Hence it follows  that  $\Phi$ is a  $C^{N_0}$-diffeomorphism from $U_0$, a small neighborhood  of $0$ in $S$, to a certain real hypersurface  of $(-1,1)\times\CC^{n}$  near $(0,0)$. Moreover, $\Phi(t,\cdot)$ is a local CR diffeomorphism. For each fixed $t$, denote by $\Psi(t,\cdot)$ the inverse CR diffeomorphism of $\Phi(t,\cdot)$.  We write $S^*_t=\Phi(t, S_t\cap U_0)$. Then $S_t^*$ is also a strongly pseudoconvex hypersurface near $\pi(p(t))$ where $p(t):=\psi(t, p^*_0)$ for a certain $p^*_0\in S_0$ is a $C^{N_0}$-smooth curve near $p_0$ such that  $p(t)\in S_t$ with $p(0)=p_0=0$. It is transversal to $S_0$.  Let $D^*_{t}$  be a small domain near $\pi(p(t))$ in the strongly pseudoconvex side of $S^*_t$ such that any point in  $D^*_{t}$  can be connected by a continuous family of embedded holomorphic disks attached to $S^*_t$ shrinking down to $\pi(p(t))$ and $D^*_{t}$ contains every point in the pseudoconvex side of $S^*_t$ that has Euclidean distance to $\pi(p(t))$ less than a certain positive constant $\e_0$.  % By the Boauendi-Treves approximation theorem of CR functions by integral against Gaussian kernels,
%{\color{red}{more details will be added here}}, we can conclude that $\Psi$ extends to a smooth function over a  small domain $\ov{\O_0^*}$ in $(-1,1)\times \CC^n$ and holomorphic for each fixed $t$ in  $\ov{\O_0^*}\cap D^*_t$, where   $\O_0^*\cap D_t^*$ contains  a certain fixed size of a small piece of $p(t)$ in  $S^*_t$  as part of its smooth boundary for $t$ with $|t|\ll1$. Write
%Since each $S^*_t$ is a $C^{N_0}$-smooth family of strongly pseudoconvex manifolds, we  see the $C^{N_0}$-smooth dependence of $\Psi(t,\cdot)$  in $t$.
%by tracing  the  proof of the Lewy extension theorem  as follows:

%\begin{lemma}\label{ope} For $|t|<\e_1\ll1$, $\Psi$ extends to a $C^{[N_0/2]-1}$-smooth function over a small domain $\ov{\O_0^*}$ in $(-1,1)\times \CC^n$ such that $\Psi(t,\cdot)$ is holomorphic over  $\O_0^*\cap D_t^*$, where   $\ov{\O_0^*\cap D_t^*}$ contains every point  in   the pseudoconvex side of ${S^*_t}$ with a Euclidean distance to $\pi(p(t))$ bounded by $0<\e_3<\e_0\ll1$. %Here we make the convention that $[N_0/2],[N_0/2]-1=\infty$ if $N_0=\infty$, and $[N_0/2],[N_0/2]-1=\omega$ if $N_0=\omega$. %Here  $\e_0,\e_1$ are both sufficiently small positive constant. 
%\end{lemma}
%The case for $N_0=\omega$ is a consequence of the classical Cartan theorem (see for instance \cite{HY3}). Hence we assume that $N_0\leq\infty$.

%\begin{proof}[Proof of Lemma \ref{ope}] We will follow the proof of the classical Lewy extension theorem (see, for instance, \cite{CS}) and study   the dependence on $t$. 

%By shrinking $U_0$ and making a  holomorphic  change in $z\in \CC^n$ that depends $C^{N_0}$-smoothly on $t$, %$\left(t^{\prime},z^{\prime}\right):=\left(t,z-\pi(p(t))\right)$, 
%we may assume that the image $M:=\Phi(S\cap U_0)$ is a hypersurface defined by a  %$C^{N_0}$-smooth function 
%\begin{equation}\label{boundary}
%r(t,z):=-\h{Re}\,z_n+\sum\nolimits_{j=1}^n |z_j|^2+r^*(z,t)=0 %z_k+\h{Re}\left(\sum\limits_{j,k=1}^n\frac{\partial^2r(t,0)}{\partial %z_j\partial z_k}z_j z_k\right)+O(|z|^3)=0,
%\end{equation}
%in a certain open subset $\widehat U$ of  $(-1,1)\times\CC^{n}$  near $(0,\pi(p_0))=(0,0)$. Here $r(z,t)=O(|z|^3)$, and $(t, p(t)$) is mapped to $(t,0)$ in the new coordinates.  
%Then, after a change of coordinates  
%$$\left(\widetilde t,\widetilde z_1,\widetilde z_2,\cdots,\widetilde %z_n\right):=\left(t,z_1,\cdots,z_{n-1}, z_n+\sum\nolimits_{i=1}^{n-1}%{a_i(t)}z_i+\sum\nolimits_{j,k=1}^n\frac{\partial^2r(t,0)}{\partial z_j\partial z_k}z_j z_k\right),$$ we may further assume that 
%\begin{equation}\label{ndf}
%r(t,z)=\h{Re}\,z_n+\sum\nolimits_{j,k=1}^n M_{j\ov{k}}z_j\ov{z_k}+r^*%(t,z),   \end{equation}
%where $(M_{j\ov{k}}(t))$ is a positive definite Hermitian matrix %depending $C^{N_0}$-smoothly on $t$, $r^*(t,z)=O(|z|^3)$ is $C^{N_0}$-%smooth on $(t,z)$. 
%Thus, we can  choose $\delta>0$, and then  $\epsilon>0$ such that $\frac{\partial^2r}{\partial z_1\overline\partial z_1}>0$ and $\frac{\partial r}{\partial z_n}\neq 0$ on 
%$$U^{\prime}:=\{(t,z)\in(-1,1)\times\mathbb C^n: |z_1|<\delta\,\,{\rm and}\,\, |t|+|z_2|+|z_3|+\cdots+ |z_n|< %\epsilon\}\subset \widehat U$$
%and that $r(t,z)>0$ on the part of the boundary where $|z_1|=\delta$. Write $U^{\prime}_{-}$ for the subset of $U^{\prime}$ where $r(t,z)<0$.
%and that $U^{\prime}$ is contained in a tubular neighborhood $ \wt{M}$ of $M$ with $R:\wt M\rightarrow M$ being the smooth retraction along $z_n$-direction. 
%Write \begin{equation*}
%{U}^{\prime}_+:=\{(t,z)\in U^{\prime}|r(t,z)>0\},\,\,{\rm and}\,\,\,  %{\overline U}^{\prime}_+:=\{(t,z)\in U^{\prime}|r(z)\geq 0\}.  
%\end{equation*}



%Now let $f(t,z)$ be a $C^{N_0}$-smooth function defined on $U^{\prime}$ such that for each fixed $t$, $f(t,\cdot)$ is a CR function in $z\in S^*_t$. Fix an $N\in \NN$ with $6\le N\le N_0$, and when $N_0<\infty$,  let $N=N_0.$ As we did in (\ref{dbar-01}), we can find $C^{[N/2]}$-smooth functions $h_1,\cdots, h_{[N/2]}$ in $(z, t)$ near $(0,0)$ such that
%$$\widetilde f(t,z)=f(t,z)-\sum\nolimits_{j=1}^{[N/2]} h_j(t,z)\cdot (r(t,z))^j$$
%has the property that %$\ov\partial_z\widetilde f(t,z)=O(r^{[N/2]})$.

%We can extend $f$ to a $C^{N_0-1}$-smooth function on $U^{\prime}$ by 
%\begin{equation*}
%\widetilde f(t,z):=(f\circ R)(t,z)-\frac{r(t,z)}%{\sqrt{\sum_{i=1}^n\left|\frac{\partial r}{\partial z_i}\right|^2}}\cdot\sum_{j=1}^n\frac{\partial}{\partial\overline z_j}\left(\frac{r(t,z)}{\sqrt{\sum_{i=1}^n\left|\frac{\partial r}{\partial z_i}\right|^2}}\right)\frac{\partial (f\circ R)(t,z)}{\partial z_j}.
%\end{equation*}
%It is clear that $\frac{\partial \widetilde f(t,z)}{\partial\overline z_i}=0$  on $U^{\prime}\cap M$, $1\leq i\leq n$. 
%Note that for any fixed %$(t,z_2,\cdots,z_n)$ in
%$$V:=\{(t,z^{\prime}):=(t,z_2,z_3\cdots,z_n)\in(-1,1)\times\mathbb C^{n-1}: |t|+|z_2|+|z_3|+\cdots+ |z_n|< \epsilon\},$$ 
%the set of all $z_1$ with $|z_1|%<\delta$ such that $r(t,z_1,z_2,\cdots,z_n)>0$ is connected. We define a $C^{[N/2]-1}$-smooth one form $g:=\sum_{j=1}^n g_j(t,z)d\overline z_j$ on $\CC \times V$ by
%$g_j(t,z):=\frac{\partial \widetilde f(t,z)}{\partial\overline z_j}$ %$$,\,\,\,\,\,\,\,\forall\, (t,z)\in,\,\,1\leq j\leq n$$
%on ${\overline U}^{\prime}_-$ and $0$ otherwise,  $1\leq j\leq n$.
%\begin{equation*}\left\{\,\begin{aligned}&g_j(t,z):=0,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\,\forall\, (t,z)\in(\mathbb C\times V)\setminus {\overline U}^{\prime}_-,\,\,1\leq j\leq n,\\&g_j(t,z):=\frac{\partial \widetilde f(t,z)}{\partial\overline z_i}d\overline z_j,\,\,\,\,\,\,\,\forall\, (t,z)\in{\overline U}^{\prime}_-,\,\,1\leq j\leq n.\end{aligned}\right. \end{equation*}
%For any $(t,z_2,z_3\cdots,z_n)\in V$, we define
%\begin{equation*}%\label{lci}
 %G(t,z_1,z_2,\cdots,z_n):=\frac{1}{2\pi i}\int_{\mathbb C}\frac{g_1(t,\xi,z_2,\cdots,z_n)}{\xi-z_1}\,d\xi\wedge d\overline \xi.  
%\end{equation*}
%We  conclude, from the fact that $g_1\in C^{[N/2]-1}$,  that $\ov\partial G=g$ and $G(t,z)\in C^{[N/2]-1}(\mathbb C\times V)$.
%\begin{equation*}\sum\nolimits_{j=1}^n\frac{\partial G(t,z)}{\partial\overline z_i}d\overline z_j=g=\sum\nolimits_{j=1}^n g_j(t,z)d\overline z_j. \end{equation*}
%in the distribution sense. 
%$G(t,\cdot)$ is holomorphic in $z$ on $(\mathbb C\times V)\setminus {\overline U}^{\prime}_-$. Also for each $(t,z_2,\cdots, z_n)\in V$, the set $\{z_1\in\mathbb C:r(t,z_1,z_2,\cdots,z_n)>0\}$  is connected, for otherwise $r$, as a function in $z_1$, achieves a minimum value where  $\frac{\partial^2r}{\partial z_1\overline\partial z_1}>0$ which is a contradiction. 
 %For a sufficiently small positive number 
%$\eta$, there is a small open neighborhood $V_0$ of %$(0,\cdots,0,\eta)\in V$ such that $\mathbb C\times V_0\subset\mathbb %C\times V$ and $r(t,z_1,\cdots,z_{n-1},z_n)>0$ on $\mathbb C\times %V_0$. We  thus easily conclude by (\ref{lci}) that  $G(t,z)\equiv 0$ on $U^{\prime}\cap M$. 
%Now the function $F=f-G$ 
%is in $C^{[N/2]-1}({\overline U}^{\prime}_-)$ with $F=f$ on $U^{\prime}\cap \mathcal M$ and $F(t,\cdot)$ is holomorphic in $z$ on $U^{\prime}$. Notice that $F$ is independent of the choice of $\wt f$.  The proof of Lemma \ref{ope} is complete. \end{proof}


%We still write $\Psi$ for its holomorphic extension.  Repeat the above procedure at sufficiently many  points  $\{p_j\}_{j=0}^m\subset  S_0$ such that the constructed $\{\ov{\O_j}:=\Psi_j(\ov{\O^*_j})\}_{j=0}^m$ covers a neighborhood of  $S_0$ in $S$.  Then there is a union of a family of mutually disjoined  complex submanifolds of codimension one $\O_{\e_4}\subset \mathcal M$ with $0<\e_4\ll1$ such that 
%$S$ near $S_0$ is  part of the $C^{[N_0/2]-1}$-smooth boundary of $\O_{\e_4}$ and $\O_{\e_4}$ stays in the pseudoconvex side of $S$, and that %$\O_{\e_1}$ contains every point in the pseudoconvex side of $S$ with a Euclidean distance to $S_0$ bounded by $\e'_1$, where $\e_1'>0$ is a small number. 
%if $x\in\cup_{t\in (-\e',\e')} \widehat S_t$ is in the pseudoconvex side of $S$ with  the distance of $x$ to $S_0$ is less than $\e''_1$ for a certain fixed metric, then $x\in \O_{\e_4}$, where $\e_1',\e_1''>0$ are small numbers. 

%Notice that $\widehat S_0$  has no singularity by the assumption. Let $\rho$ be a $C^{[N_0/2]-1}$-smooth defining function of $S$ near $S_0$ in $\ov\O_{\e_1}$, that is  strongly plurisubharmonic when restricted to $\wh{S_t}$  for $|t|\ll1$. it  also vanishes   on $S_t$ for $|t|\ll1$.  Write in what follows for any $0<\e_j\ll1$ with $j=5,6$, 
%\begin{equation}\label{noboundary}
%\wh{S}_{t,\e_j}:=\{z\in \wh{S}_t:  \h{ either }z\not\in \O_{\e_1} \h { or } \rho(z)<-\e_j\}.    
%\end{equation}
%According to a result of Stein (see \cite[Theorem 3.3.3]{Fo} for instance), there is a holomorphic retraction $R$ from a neighborhood $V$ of   $\wh{S}_{0}$ in $\mathcal M$
%to  $\wh{S}_{0}$ with the retraction along the complex normal direction of  $\wh{S}_{0}$. Also in a certain small local chart at any $z_0\in \wh{S_0}$, $R$ can be written as the projection to its first $n$-components.  Let $0<\epsilon_5\ll\e_1$. It is clear that for $|t|\ll1$, the restriction $R(t,\cdot)$ of $R$ to $\wh{S}_{t, \e_5}$ maps $V\cap \wh{S}_{t, \e_5}\cap \O_{\e_1}$ biholomorphically to a complex open submanifold $E_{t,\e_5}$ of $\wh{S}_{0}$.  Notice that the outer boundary of $E_{t,\e_5}$ %,  denoted by $\wh{S}_{0, t,\e_2}$, 
%is strongly pseudoconvex.   %
%$\wh{S}_{0, t,\e_2}$ 
 %slightly to $\wh{S}_{0, \e_4}$ with $\e_4>\e_2$,
%Letting $\e_6>\e_5$, we have $\p \wh{S}_{0, \e_6}\subset E_{t,\e_5}$ for any $-\e'<t<\e'$ with $0<\epsilon'\ll1$.

%$$\frac{\partial^2r}{\partial z_1\overline\partial z_1}>0$$
%Now, let $0<\e_2\ll\e_1$ and write
%$\wh{S}_{0,\e_2}$ for the part of $\wh{S}_{0}$ such that  $\wh{S}_{0,\e_2}$ is Stein,  $\p\wh{S}_{0,\e_2}\subset \O_{\e_1}$ and $\p\wh{S}_{0,\e_2}$ is within the distance $\e_2$ to $S_0$. By shrink $\epsilon_2$, $\epsilon_3$, we may assume that $E_{t,\e_1}$ contains $\p\wh{S}_{0,\e_2}$ for any  $-\epsilon_3<t<\epsilon_3$.


%Then we  apply the Hartogs extension theorem to the inversion $(R(t,\cdot))^{-1}$ to get a map $H(t,z):=(h_1(t,z),h_2(t,z),\cdots, h_{n+1}(t,z))$ on $(-\e',\e')\times \wh{S}_{0,\epsilon_6}$ such that
%\begin{enumerate}[label=(\roman*)]
%\item $h_i(t,z)$ is holomorphic in $z$ for  $1\leq i\leq n+1$ and $(t,z)\in(-\e',\e')\times\wh{S}_{0,\epsilon_6}$ and $H(t,z)$ has full rank near the  boundary of $\wh{S}_{0,\epsilon_6}$;
    
%\item $h_i(t,z)$ is $C^{[N_0/2]-1}$-smooth in $(t,z)$ for all $1\leq i\leq n$ and $(t,z)$ in 
%\begin{equation}\label{bd}
%\{(t,z):-\e'<t<\e',\,\,z\in (\wh{S}_{0,\epsilon_5}\cap\Omega_{\epsilon_1})\}. %\cup E_{t,\epsilon_5}\}.
%\end{equation}
%\end{enumerate}

%$H$ depends biholomorphically on $p\in \wh{S_0}_{\e_2}$ and smoothly on $(t,p)$. {\color{red}{will add more details here}} 

%\begin{lemma}\label{hsm}
%$H(t,z)$ is a $C^{[N_0/2]-1}$-%smooth map on $(-\e',\e')\times \wh{S}_{0,\epsilon_6}$. 
%\end{lemma}    
%\begin{proof}[Proof of Lemma \ref{hsm}]
%In what follows, we shall prove by induction on $k\le [N_0/2]-1$ that $h_i(t,z)'s$ are 
%$C^k$-smooth in $(t,z)$ for all $(t,z)\in(-\e',\e')\times\wh{S}_{0,\epsilon_6}$ for $1\leq i\leq n$. %For convenience, we denote $h_i(t,z)$ by $h(t,z)$.

%Fix an arbitrary point $(t,z)\in(-\e_3,\e_3)\times\wh{S}_{0,\epsilon_2}$. Take $0<\epsilon_2^{\prime}<\epsilon_2$ such that 


%By the Bochner-Martinelli formula (see, for instance, \cite[Theorem 4.3.3]{HEGE}),  for any holomorphic function $f(z)$ on $\wh{S}_{0,\epsilon_6}$ that is continuous on $\ov {\wh{S}_{0,\epsilon_6}}$, we have that
%\begin{equation}\label{bm}
%f(z)=\int_{\xi\in\partial \wh{S}_{0,\epsilon_6}}f(\xi)\cdot\psi(z,\xi)\cdot\Omega(z,\xi),\,\,\, \forall\,z\in\wh{S}_{0,\epsilon_6}.
%\end{equation}
%Here $\Omega(z,\xi)$ is a certain $C^{\infty}$-smooth section in the pull-back of the bundle $\wedge^{2n-1} T^*(\wh{S}_{0,\e_5})$ with respect to the map $\wh{S}_{0,\e_5}\times \wh{S}_{0,\e_5}\ni(z,\xi)\mapsto z\in \wh{S}_{0,\e_5}$, that is, a $C^{\infty}$-smooth $(2n-1)$-form in $\xi$; $\psi(z,\xi)$ is a certain at least $C^2$-smooth function on $(\wh{S}_{0,\e_5}\times \wh{S}_{0,\e_5})\setminus\{(z,z)|z \in \wh{S}_{0,\e_5}\}$ (see \cite[Lemma 4.2.4]{HEGE}).
%Setting $f=h_i(t,z)$ in (\ref{bm}), it is clear that $h_i(t,z)$ is continous on $(-\e',\e')\times \wh{S}_{0,\epsilon_6}$. Taking its $t$-derivative, we derive that 
%\begin{equation}\label{cau}
%\frac{\partial h_i(t,z)}{\partial t}=\int_{\xi\in\partial \wh{S}_{0,\epsilon_6}}\frac{\partial h_i(t,\xi)}{\partial t}\cdot\psi(z,\xi)\cdot\Omega(z,\xi),\,\,\,\forall\,(t,z)\in(-\e',\e')\times\wh{S}_{0,\epsilon_6},
%\end{equation}
%and hence $\frac{\partial h_i(t,z)}{\partial t}$ is continuous on $(-\e',\e')\times \p\wh{S}_{0,\epsilon_6}$ by 
%property (ii).  

%For any $z\in\wh{S}_{0,\epsilon_6}$, in a local holomorphic chart, take a polydisc $B(\eta_1,r)\times B(\eta_2,r)\times\cdots\times B(\eta_n,r)\subset\wh{S}_{0,\epsilon_6}$ containing $z$. Since $h_i(t,z)$ is holomorphic in $z$, the Cauchy integral formula yields that for any $t\in(-\e',\e')$,
%\begin{equation}\label{hol-001}
%\begin{split}
%h_i(t,z_1,\cdots,z_n)=\frac{1}{2\pi i}\int_{|\xi_n-\eta_n|=r}\cdots\int_{|\xi_n-\eta_n|=r} \frac{h_i(t,\xi_1,\cdots,\xi_n)}{(\xi_1-z_1)\cdots(\xi_n-z_n)} d\xi_1\cdots d\xi_n.   
%\end{split}    
%\end{equation}
%Differentiating (\ref{hol-001}) with respect to $t$, we conclude that $\frac{\partial h_i(t,z)}{\partial t}$ is holomorphic in $z$ for $(t,z)\in(-\e',\e')\times \wh{S}_{0,\epsilon_6}$.  Also in a local chart $\wh{S}_{0,\epsilon_6}$ with holomorphic coordinates still denoted by $z$,  $\frac{\partial h_i(t,z)}{\partial z_j}$ is continuous in $(t,z)$. Therefore, we showed that $h(t,z)$ is  $C^1$-smooth in its variables. 

%Suppose that $h_i(t,z)$ is $C^{k^{\prime}}$-smooth in $(t,z)$ for all $1\leq k^{\prime}<k$ and $(t,z)\in(-\e',\e')\times\wh{S}_{0,\epsilon_6}$. We proceed to show that $h_i(t,z)$ is $C^{k^{\prime}+1}$-smooth for all $(t,z)\in(-\e',\e')\times\wh{S}_{0,\epsilon_6}$. 

%Notice that for any holomorphic vector field $\mathcal D$ on $\wh{S}_{0,\epsilon_5}$, $\mathcal D(h_i)(t,z)$ is holomorphic in $z$. By setting $f=\mathcal D(h_i)(t,z)$ in (\ref{bm}), we can further conclude by property (ii) that $\mathcal D(h_i)(t,z)$ is continuous on $(-\e',\e')\times \wh{S}_{0,\epsilon_6}$. %and continuous for $(t,z)\in(-\e_3,\e_3)\times\wh{S}_{0,\epsilon_4}$. 
%Now assume that it is $C^{k-1}$-smooth in $(t,z)$. 
%Since any $z$-derivative at $(t,z)\in(-\e',\e')\times \wh{S}_{0,\epsilon_5}$ is generated by a holomorphic vector field on $\wh{S}_{0}$ by Cartan's Theorem A,  it suffices to prove that $\mathcal D_{k^{\prime}+1}(\mathcal D_{k^{\prime}}\cdots(\mathcal D_1(h_i)))$
%is continuous on $(-\e',\e')\times \wh{S}_{0,\epsilon_6}$, where each $\mathcal D_j$, $1\leq j\leq k^{\prime}+1$, is either $\frac{\partial}{\partial t}$ or a holomorphic vector field defined on $\wh{S}_{0}$. By induction, $\mathcal D_{k^{\prime}}\cdots(\mathcal D_1(h_i))$ is holomorphic in $z$ for $(t,z)\in(-\e',\e')\times\wh{S}_{0,\epsilon_6}$, and $C^{[N_0/2]-1-k^{\prime}}$-smooth in $(t,z)$ for $(t,z)$ in (\ref{bd}). By the same argument as above, we  see that $\mathcal D_{k^{\prime}+1}(\mathcal D_{k^{\prime}}\cdots(\mathcal D_1(h_i)))$ is continuous on $(-\e',\e')\times \wh{S}_{0,\epsilon_6}$. 

%The proof of Lemma \ref{hsm} is complete.\end{proof}


%Next we proceed to prove that $\widehat S$ is a $C^{[N_0/2]-1}$-smooth real hypersurface near $\widehat S_0$. 

%We claim that the Jacobian matrix of map $H(t,z)$ is of full rank, when $t=0$ and $z\in\wh{S}_{0,\epsilon_6}$. Otherwise, assume that $H(t,z)$ is degenerate at $(0,z^*)$ with $z^*\in\wh{S}_{0,\epsilon_6}$. We take local coordinates $(z_1,z_2,\cdots,z_{n+1})$ in a neighborhood of a point $H(0,z)\in\mathbb C^{n+1}$ with $z\in\wh{S}_{0,\epsilon_6}$ such that  $$H(0,z_1,z_2,\cdots,z_n)=(h_1(0,z_1,z_2,\cdots,z_n),\cdots, h_{n+1}(0,z_1,z_2,\cdots,z_n))\equiv(z_1,\cdots,z_n,0).$$ 
%Then computation yields that $H$ is degenerate at $(0,z)$ if and only if $\frac{\partial h_{n+1}(t,z)}{\partial t}|_{t=0}=0$. Since $\frac{\partial h_{n+1}(t,z)}{\partial t}|_{t=0}$ is holomorphic in $z$ as shown above, we conclude that the degenerate locus $\mathcal J:=\{z\in\wh{S}_{0}:H{\rm\,\, is\,\, degenerate\,\, at\,\,}(0,z)\}$
%is a nonempty complex analytic subvariety of $\widehat S_0$ of codimension one. Then $\mathcal J$ must intersect $S_{0,\e_5}$, for $\dim_{\mathbb C}\mathcal J\geq1$ and $\wh S_0$ is Stein,  which is a contradiction.


%By the uniqueness of holomorphic functions, for $|t|<\e_3$ and $z\in \wh{S}_{0,\e_2}$, $R\circ H(t,z)=z$ as it holds  near $\wh{S}_{0,\e_4}$. Hence, we see that $H(t,z)$ must have full rank $n$. Then, for $|t|\ll1$, $H(t,z)$ must be one-to-one  as $H(0,z)\equiv z$. This shows that  $\widehat S_{t}$ is a Stein submanifold 

%Then for $|t|<\e_7$ with $0<\e_7\ll1$, $\widehat S=\cup_{t\in (-\e,\e)} \widehat S_t$ is the image of a $C^{[N_0/2]-1}$-smooth diffeomorphism and thus is a real hypersurface with the same smoothness. Also the function which assigns points in $\wh{S_t}$ to $t$ is $C^{[N_0/2]-1}$-smooth on $\wh{S}$ and $dt|_{\wh{S}}\not =0.$
%This completes the proof of Theorem \ref{openness} when $N_0\le \infty$.
%\smallskip


%When $N_0=\omega$,
%all $h_i(t,z)$ are real analytic in $(t,z)$ on (\ref{bd}). To prove that $H(t,z)$ is real analytic on $(-\e^{\prime},\e^{\prime})\times \wh{S}_{0,\epsilon_6}$, we can complexify $h_i(t,z)$ and then apply the Hartogs extension on 
%\begin{equation*}
%\left\{(\widehat t,z):|\widehat t|<\e^{\prime},\,\,z\in (\wh{S}_{0,\epsilon_5}\cap\Omega_{\epsilon_1})\right\}.
 %\end{equation*}




%. In terms of the real coordinates, we have \textcolor{red}{???}\begin{equation}\begin{split}&\left.\left(\begin{matrix}\frac{\partial{\rm Re}h_1(t,z)}{\partial t}&\frac{\partial{\rm Im}h_1(t,z)}{\partial t}&\cdots&\frac{\partial{\rm Re}h_{n}(t,z)}{\partial t}&\frac{\partial{\rm Im}h_{n}(t,z)}{\partial t}&\frac{\partial{\rm Re}h_{n+1}(t,z)}{\partial t}&\frac{\partial{\rm Im}h_{n+1}(t,z)}{\partial t}\\\frac{\partial{\rm Re}h_1(t,z)}{\partial x_1}&\frac{\partial{\rm Im}h_1(t,z)}{\partial x_1}&\cdots&\frac{\partial{\rm Re}h_{n}(t,z)}{\partial x_1}&\frac{\partial{\rm Im}h_{n}(t,z)}{\partial x_1}&\frac{\partial{\rm Re}h_{n+1}(t,z)}{\partial x_1}&\frac{\partial{\rm Im}h_{n+1}(t,z)}{\partial x_1}\\\cdots&\cdots&\cdots&\cdots&\cdots\\\frac{\partial{\rm Re}h_1(t,z)}{\partial y_n}&\frac{\partial{\rm Im}h_1(t,z)}{\partial y_n}&\cdots&\frac{\partial{\rm Re}h_{n}(t,z)}{\partial y_n}&\frac{\partial{\rm Im}h_{n}(t,z)}{\partial y_n}&\frac{\partial{\rm Re}h_{n+1}(t,z)}{\partial y_n}&\frac{\partial{\rm Im}h_{n+1}(t,z)}{\partial y_n}\end{matrix}\right)\right|_{t=t^*}\\&\,\,\,\,\,\,\,=\left(\begin{matrix}*&*&\cdots&*&*&\frac{\partial{\rm Re}h_{n+1}(t^*,z)}{\partial t}&\frac{\partial{\rm Im}h_{n+1}(t^*,z)}{\partial t}\\1&0&\cdots&0&0&0&0\\\cdots&\cdots&\cdots&\cdots&\cdots&\cdots&\cdots\\0&0&\cdots&0&1&0&0\end{matrix}\right). \end{split} \end{equation}

%The proof of Theorem \ref{openness} is complete. \end{proof}

%\begin{remark}  We remark that the regularity of $\wh{S}$ up to the boundary could be improved at least to $C^{N_0-1}$ by applying the Baouendi-Treves approximation theorem. However, for simplicity of exposition, we will be content with the $C^{[N_0/2]-1}$-smoothness of $S$, which is good enough for the proof of Theorem \ref{maintheorem-global}   as we do lose about half of the regularity near  CR singular points. (See Remark \ref{optimal-001}.) 
%\end{remark}
%. Write ${\cal S}$ for the set of CR singular points of $M$
%near $0$. Suppose that $0$ is not an isolated point in ${\cal S}$.
%Notice that $T^{(1,0)}_{0}M=\hbox {span} \{\frac{\p }{\p
%z_1}|_0,\cdots, \frac{\p }{\p z_n}|_0 \}$. For $p_0\in {\cal S}$
%close to $0$, we easily see that  $T^{(1,0)}_{p_0}M=\hbox {span}
%\{X_1,\cdots, X_n\}$ for certain  tangent vectors of type $(1,0)$ of
%the form: $X_j=\frac{\p }{\p z_j}|_{p_0}+b_j\frac{\p }{\p
%w}|_{p_0}$, $j=1,\cdots, n$. Since $X_j(\ov{-w+q+F})=0$,  we get
%$\ov{z_j}+2\lambda_j{z_j}=O(|z|^2)$ when $q_0\approx 0$. Write
%$z_j=x_j+\sqrt{-1}y_j$. Then $(1+2\lambda_j)x_j=O(|z|^2),
%(1-2\lambda_j)y_j=O(|z|^2)$ for $j=1,\cdots, n$. By the implicit
%function theorem,
% we conclude that
%if $\lambda_j\not = \frac{1}{2}$, we must have $z_j=0$. When
%$\lambda_j=\frac{1}{2}$, we must have $x_j=0$.  In any case
%${\cal S}$ is contained in a submanifold of $M$ near $0$ which has
%at most real dimension $n$; and when none of the Bishop invariants
%of $M$ at $0$ is parabolic, the only CR singular point of $M$ near
%$0$ is $0$ itself.
